PromptPath: Prompt-Adaptive Computational Pathways for In-Context Learning

In-context learning (ICL) has attracted increasing attention for enabling models to perform new tasks using only a few ``input--output'' prompt examples. However, existing approaches suffer from \textbf{shallow task adaptation}, where prompts are primarily used as contextual cues to implicitly infer task intent through semantic representations, while the underlying computational process remains unchanged. This limitation restricts task-specific adaptation and compromises inference interpretability. We argue that prompts should not only condition feature representations but also dynamically regulate the model's computation pathways. To this end, we propose \textbf{PromptPath}, an adaptive ICL framework that enables computation-level adaptation through prompt-conditioned dynamic pathways. Specifically, PromptPath introduces a prompt-driven routing mechanism to selectively activate and compose lightweight low-rank experts, forming task-specific computational pathways tailored to different prompts. By integrating prompt information directly into the inference process, PromptPath dynamically reconfigures model computation to enhance task specialization and interpretability. Extensive experiments on 3D point cloud and 2D visual recognition benchmarks demonstrate that PromptPath consistently outperforms state-of-the-art ICL baselines while exhibiting strong cross-domain and cross-task generalization.

==> sec/6_discussion.tex <==
\clearpage
\setcounter{page}{1}

\setcounter{table}{0}
\renewcommand\thetable{A\arabic{table}}
\setcounter{figure}{0}
\renewcommand{\thefigure}{A\arabic{figure}}  

% \maketitlesupplementary
\section{Discussion}

\subsection{\textbf{Limitations}}

Although PromptMoE achieves comprehensive improvements over a wide range of state-of-the-art baselines, its qualitative results may still exhibit occasional inaccuracies in certain complex and challenging cases. We hypothesize that this may stem from the remaining room for hyperparameter refinement. For example, the LoRA rank used in the Low-Rank Expert Library may benefit from larger values; however, our experiments were currently limited to a maximum rank of 32 due to computational constraints.



\subsection{\textbf{Broader Impacts}}

This work presents PromptMoE, a novel computation level in-context adaptation framework that enables models to highly dynamically reorganize their internal processing pathways based on task prompts. By making task-dependent computation explicit and interpretable, PromptMoE has the potential to influence several promising research directions. In particular, it may stimulate new developments in adaptive vision systems, modular neural architectures, and resource-efficient multi-task learning—especially in settings where accommodating diverse tasks without fine-tuning is absolutely critical. More concretely, by extending in-context learning from representation-level conditioning to computation-level adaptation, PromptMoE offers foundational insights that may reshape how adaptive reasoning is designed for visual intelligence.
